Mining User Opinions in Mobile App Reviews: A Keyword-based Approach

User reviews of mobile apps often contain complaints or suggestions which are valuable for app developers to improve user experience and satisfaction. However, due to the large volume and noisy-nature of those reviews, manually analyzing them for useful opinions is inherently challenging. To address this problem, we propose MARK, a keyword-based framework for semi-automated review analysis. MARK allows an analyst describing his interests in one or some mobile apps by a set of keywords. It then finds and lists the reviews most relevant to those keywords for further analysis. It can also draw the trends over time of those keywords and detect their sudden changes, which might indicate the occurrences of serious issues. To help analysts describe their interests more effectively, MARK can automatically extract keywords from raw reviews and rank them by their associations with negative reviews. In addition, based on a vector-based semantic representation of keywords, MARK can divide a large set of keywords into more cohesive subsets, or suggest keywords similar to the selected ones.

==> background.tex <==



==> crawler.tex <==



==> future.tex <==
Future work

- Summarization of reviews $rightarrow$ better represent common opinions!

- Common concerns for different categories of mobile apps (by pre-defined keyword sets).

- Comparative mining of user opinions in two apps $rightarrow$ help customers, app developers!

==> introPhong.tex <==
\section{Introduction}
As the use of mobile devices such as smartphones and tablets explodes, developing software applications (i.e. often called apps) for those devices is becoming a highly popular and profitable business in software development. However, it is also a highly competitive business, as millions and counting apps of different categories are available on major app markets like Apple App Stores or Google Play. Since revenue and profit of mobile apps are often proportional to the size of their userbases, improving user satisfaction to retain existing users and attract new ones is of important to app developers.

To improve user satisfaction, mobile app developers could rely on relevant user opinions such as complaints or suggestions. As most online app markets provide a rating and reviewing mechanism for users of mobile apps, user reviews on app markets provide an important source for such opinions. However, manual analysis of those reviews for useful opinions is often challenging. First, due to the sheer size of its userbase, a popular apps (with million users) often gets thousands reviews each day. In addition, not all reviews worth reading. Prior research reports that more than 60\% of reviews are noise, i.e. do not contain useful opinions~\cite{Chen:2014:AMI:2568225.2568263}.

%In such competitive environment, app developers have to make their apps more appealing to users in order to stay on their business. That means their apps must meet user's expectation. Most App Markets provide a rating and reviewing system as an interface for users to reach out to app developers by inputing their rating of the apps or telling their opinions and concerns. Developers need to gather these information and change their apps accordingly to keep their customers. However, popular apps that have millions of users also receive millions of such reviews from them overtime. It is extremely resource inefficient for developers to read all of those reviews. More than that, only a small fraction of them contains useful information and many others are just not worth reading. This poses the problem of mining useful opinions from user's reviews.



We assume that both developers and users often express their concerns via some keywords. For example, they can describe their concern about battery consumption with keywords like "battery", "hog", "drain", "overheat". If a review contains most of these keywords, it is likely that it describe the concern. Following this intuition, we propose \tool  Framework to extract the keywords that represent user's concerns from app reviews and prompt the most important ones to developers. To rank the keywords, we first find the alignment between good and bad of each keywords by calculating the ratio between the number of time a keyword appears in reviews with bad rating to the number of time it appears in the ones with good rating. This ratio score is then pushed further with the difference between number of good and bad ratings to measure its impact on the majority of users. In the end, the final score will be able to determine how good/bad a keyword is and how much impact does it have.

More than that, a concern could be expressed by not just one keywords, as for the battery consumption problem stated above. This leads to the need of developers to group the available keywords into smaller subsets, each of which describes a more general concern. We use Word2vec \cite{DBLP:journals/corr/abs-1301-3781} tool to find the vector space representations for each keywords, then apply K-mean Clustering (\notice{Cite this thing}) to group many keywords together into clusters that describe common user's concern. Following our evaluation, this grouping method reached 77\% in average accuracy.

Another common practice of users is to describe a single concern by many different keywords. In the context of app reviews, those keywords could bear similar meaning to some extent and should not be discriminated. We assume that developers may want to find the reviews of all of these keywords to further understand user's opinions. To address this problem, we use the vector base representation learned from keywords and find the keywords that has similar meaning or close relationship with a set of given words. To compare the vectors, we apply Cosine Similarity  (\notice{Cite this thing})  on them. On average, our technique achieves 89\% accuracy.

Prior studies \cite{Chen:2014:AMI:2568225.2568263}\cite{Fu:2013:WPH:2487575.2488202} also observed that the opinions of user may change overtime for an app. One example is after each release, users may start to talk about new problems of new features, or stop talking about an old problem because it had been solved. To discover this trend, we apply Moving Average (\notice{Cite this thing}) on keyword's timeseries to find the sudden changes in keywords occurrence overtime. These changes give an insight of when a big concern appeared and when it is solved. Our evaluation shows that this technique can actually point out the trends that were addressed by actual developers.

The keywords can help describe opinions, concerns, but they alone without context would not suffice for a complete understanding. Developers need to read the actual reviews of the concerns, but only the most important ones. To provide them with most informative reviews, we rank the reviews accord to the set of keywords that developers want. In our ranking schema, each keyword may have difference level of importance in the whole picture. If a keywords is mentioned almost every time users input their reviews, then it is likely not a good keyword at all. Vice versa, if a keyword is only mentioned in a selected set of reviews, then those reviews should be talking about a specific concern relate to that keyword. We use TFIDF technique (\notice{Cite this thing}) to rank such keywords and then calculate Cosine Similarity on TFIDF between the keywords set and the reviews. The final score will be used to rank the most informative reviews.

Finally, we evaluate our approaches using over 2 millions reviews crawled for more than four months on Google Play. This paper is structured as follows: Section 2 explains the background knowledge for our approach, Section 3 describe the \tool framework, Section 4 describes our methods to preprocess review's data, Section 5 explains our approaches for mining keywords. Section 6 explains our Trends detector and Section 7 evaluates our approaches. Lastly, we discuss on related works and then conclude our study.


==> temp.tex <==




\subsubsection{Data storage and Vector-based representations}\label{sec:storing}

In \tool, we have a step of grouping keywords to find common concerns among them. To do such task, we need to find words with common meanings or relationships and put them together. Simple statistical models such as topic modeling \cite{LDA} can capture topics based on the frequency of a word in different documents, however, it is not intended to capture semantic regularities of words. Recent studies on vector-space distributed representation of words had suggested that words can have multiple degrees of similarity \cite{mikolov2012statistical}. Exploiting this property of word vectors could help us to group semantically similar keywords together. We discuss more on this in Section \ref{sec:dividing}. In our work, we use Word2vec tool to learn the vector-representations of words and store them in a database for later use.

After normalization step, in every app, we count the occurrence of each keyword over time for each rating level. This information can be later used to rank keywords and analyze their trends. The time unit is day, thus each word will have 5 vectors of daily occurrences for five rating levels. It is also relatively simple to just update the daily occurrences when new reviews arrive. The following definitions explain how we store our data:

\begin{myitemize}
	  \vspace*{-0.5\baselineskip}
\item $A = \{a_1, a_2, ..., a_N\}$ is a discrete set of $N$ vocabularies for $N$ apps from app stores.
\item $a_i = \{w_1, w_2, ..., w_k \}$ is a set of $k$ keywords found in reviews of $a_i$
\item $w_k = \{v, D\}$ where $v$ is the vector-based representation of $w_k$ AND $D = \{r_1, r_2, r_3, r_4, r_5\}$ contains word counts $r_x$ for 5 each rating level, $r_x =\{d_1, d_2, ..., d_j \}$ contains count for each day of $j$ days.
\end{myitemize}


The


\begin{definition}
Given a keyword vocabulary $V$, an importance measure $\lambda$, return all keywords $u \in V$ in descending order of $\lambda(u)$.
\end{definition}
	
From the review's information, we know that the ratings associated with user's reviews is a measurement for sentiment of that reviews. At keyword level, if many users decide to give low ratings to reviews contain a particular keyword, that keyword could expresses the feature that they are concerning about. Through manual inspection of 400 reviews chosen randomly in our dataset, we found that users often use the same terms on the reviews that talk about the same topic. For example,

	% Table generated by Excel2LaTeX from sheet 'Sheet1'
	\begin{table}
	  \centering
	  \sf
	  \renewcommand{\arraystretch}{0.6}
	  \caption{The intersection of negative-aligned words between three methods, tested on dataset described in section \ref{sec:data}}
	    \begin{adjustbox}{max width=0.5\textwidth}
	    \begin{tabular}{|c|c|c|c|}
	    \hline
	    \textbf{} & \textbf{Pearson} & \textbf{Sknewness} & \textbf{Contrast} \bigstrut\\
	    \hline
	    \textbf{Pearson} & -     & 96\%  & 96\% \bigstrut\\
	    \hline
	    \textbf{Skewness} & 98\%  & -     & 99\% \bigstrut\\
	    \hline
	    \textbf{Contrast} & 98\%  & 99\%  & - \bigstrut\\
	    \hline
	    \end{tabular}%
	
	      \end{adjustbox}
	  \label{tab:intersection}%
	  \vspace*{-\baselineskip}
	\end{table}%
	
To discover the relationship between ratings and keywords, we propose a simple contrast ranking technique using just ratio and the difference between positive and negative rating counts of keywords (Equation \ref{eq:ratio}). This technique is relatively faster and simpler than the commonly used Skewness \cite{oehlert2000:statbook} or Pearson Correlation\cite{walpole1993probabilitybook} which are widely used. Pearson Correlation put more weight on too high or too low ratings, thus it is more susceptible to the influence of outliers. This complication is not needed since rating of 2 and 1 are both negative ratings (or 4 and 5 for the positive side) so we do not need to discriminate them. Skewness scoring technique, on the other hand, calculates the moment coefficients of rating counts ranging from 1 to 5. It can be used to express the negative/positive alignment of keywords but it also has to constantly calculate sample third central moment and cubic of sample standard deviation, which requires a lot of computational effort.

Our simple technique can overcome those setbacks by only taking the contrast of negative/positive counts in consideration. This contrast score includes: the ratio between negative ratings and positive ratings counts to discover negative/positive alignments; the difference between those counts to reflect the impact of the concern to users. This is because we assume that if a concern affect users more than other concerns, then they would mention its keywords more frequently in their reviews.
	
	  \vspace*{-\baselineskip}
	\begin{equation}
	Cm = (N_n - N_p) \times \tfrac{N_n}{N_p}
	\label{eq:ratio}
	\end{equation}
	\begin{myitemize}
	\item $N_n$: Number of reviews below rating 3
	\item $N_p$: Number of reviews above rating 3
	  \vspace*{-0.5\baselineskip}
	\end{myitemize}

	
To evaluate if our simple contrast score can classify positive and negative keywords as well as Pearson Correlation and Skewness, we compute the intersection between keywords with negative alignment of the three methods as shown in Table \ref{tab:intersection}. Overall, there is no significant different between the classification capability of our techniques versus the others.

\subsubsection{Abnormalities Discovery}\label{sec:evalts}
	
To evaluate our abnormalities detection technique on time-series, we use the Keywords Expanding tool to obtain a set of keywords that relate to the word ``battery'' in Facebook Messenger app the manually choose the keywords that represent the \emph{battery consumption} concern the most. In the end, our set of keywords contains: \code{``heat'', ``hog'', ``usage'', ``consumption'', ``consume'', ``battery'', ``drain'', ``hogger'', ``overheat'', ``eater'', ``eat'', ``drainer'', ``power''}. Figure \ref{fig:trendeval}(a) shows the time-series and moving average for this set over the time period of January 2015 to early May 2015.
	
The reason why we choose this concern is because of an observed complaining trend about battery consumption in early February. Our further investigation lead to a confirmation from a developer at Facebook that it was a syncing issue on Android that affect people's battery life and an update was soon brought on 13th February to address this problem\footnote{http://androidforums.com/threads/facebook-messenger-battery-drain.902687/}. Our time-series also shows a big spike during those days and the trend went normal again after the release date.
	
In the scope of this study, we suggest developers set threshold for ratio score at 2, however, it is up to them to set a more suitable threshold. Figure \ref{fig:trendeval}(b) shows that the ratio score during 12th and 13th of February raised far excess our threshold of 2 while 119 other days could not pass it. If this threshold was chosen, developers of Facebook would be able to discover this trend and address the problem without having to read through all reviews or search for the unknowns on online forums.

\subsubsection{Reviews Searching}

